Dynamically Acquiring Text Content to Enable the Classification of Lesser-known Entities for Real-world Tasks

Existing Natural Language Processing (NLP) resources often lack the task-specific information required for real-world problems and provide limited coverage of lesser-known or newly introduced entities. For example, business organizations and health care providers may need to be classified into a variety of different taxonomic schemes for specific application tasks. Our goal is to enable domain experts to easily create a task-specific classifier for entities by providing only entity names and gold labels as training data. Our framework then dynamically acquires descriptive text about each entity, which is subsequently used as the basis for producing a text-based classifier. We propose a novel text acquisition method that leverages both web and large language models (LLMs). We evaluate our proposed framework on two classification problems in distinct domains: (i) classifying organizations into Standard Industrial Classification (SIC) Codes, which categorize organizations based on their business activities; and (ii) classifying healthcare providers into healthcare provider taxonomy codes, which represent a provider's medical specialty and area of practice. Our best-performing model achieved macro-averaged F1-scores of 82.3% and 72.9% on the SIC code and healthcare taxonomy code classification tasks, respectively.

==> latex/sections/abstract.tex <==
 Named entities are central to many real-world applications, yet the information required for a specific task is often missing from existing knowledge resources. Our research proposes a framework that categorizes entities for a specific task given only their names as input, without requiring access to a pre-collected text corpus or structured knowledge base. Our framework uses a search engine and large language models (LLMs) to automatically acquire task-specific descriptive text, which is then paired with labeled entities to train a text-based classification model. Our results show that the models produced by our framework yield good results for classifying organization entities into 27 Standard Industrial Classification (SIC) code \footnote{The U.S. government established Standard Industrial Classification (SIC) codes to classify organizations based on the activities they serve and operate within.} categories.
 % Furthermore, we can achieve high precision by applying confidence-based thresholding, enabling automated knowledge population with strong integrity.
 % and minimal human intervention.

==> latex/sections/experimentsAndResultsAnalysis.tex <==
% We present our experimental results across models and input configurations, highlighting key findings and insights derived from these evaluations.

%\subsection{Prompting Baselines}
%As a baseline, we have used two different prompting strategy that we describe in section \S~\ref{sec:prompting}. The result is shown in the Table \ref{tab:gpt_performance}.

In this section, we report the results of experiments on the SIC  code classification task. We evaluate performance with respect to Precision (P), Recall (R), and F1 score, which are macro-averaged across the 27  categories.

\subsection{Prompting Experiments}
\label{sec:prompting_noContext}
As a baseline, we experimented with prompting to determine whether state-of-the-art LLMs can effectively assign SIC categories to organizations. We used the \GPTFourMini{}\footnote{We used gpt-4o-mini-2024-07-18 for these experiments.} language model for these experiments because of its strong performance–efficiency trade-off and suitability for large-scale prompting experiments at low cost.
The prompt was: \textit{``Provide only the SIC code (no descriptive text) for the organization `{ORG\_NAME}'. Just the number.''} We explicitly instructed the model to return only the SIC number without accompanying text to simplify automatic evaluation. This prompt relies solely on the LLM's internal knowledge to produce an answer, which is important to assess whether the LLM may have seen organizations' SIC codes in its pre-training data. 

% \subsection{Prompting with Context}
% \label{sec:promptingWithContext}
We also prompted the \GPTFourMini{} model with our acquired text as additional context. This prompt was: \textit{``Given the description \{DESCRIPTION\_TYPE\}, provide only the SIC code for the organization ORG\_NAME. No additional explanation needed, just the number.''}, where \texttt{ORG\_NAME} is replaced with the name of the organization. This experiment assesses whether the acquired  text can improve the LLM's prompting performance. We conducted evaluations with three types of acquired text: \GSnip{}, \SummaryGPT{}, and \SummaryLLaMA{}. %Using \SummaryGPT{} improved the F1 score to 0.546, an 8\% increase over the no-context baseline. Remarkably, incorporating \GSnip{} resulted in a significant gain, boosting the F1 score to 0.645, nearly 18\% higher than the baseline. These findings indicate that prompting alone is insufficient, whereas augmenting the prompt with retrieved text, especially Google snippets, substantially improves performance.
 
% \subsection{ Results and Analysis}
% \label{sec: resultsAnalysis}
% We evaluated the performance of our classification models, ranging from prompting to prompting with context, as well as four fine-tuned LLMs under various input configurations.
%................................................................
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{0.95}
\setlength{\tabcolsep}{2.6pt} % slightly reduced spacing

\resizebox{\columnwidth}{!}{  % ensures perfect fit in one column
\begin{tabular}{@{\extracolsep{2pt}}lrrrrrr}
\toprule
Setting & \multicolumn{3}{c}{SIC Code} & \multicolumn{3}{c}{Healthcare Taxonomy} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& P & R & F1 & P & R & F1 \\
\midrule
Prompting & 0.596 & 0.445 & 0.468 & 0 & 0 & 0 \\
\midrule
Prompting w/ \\[-1pt]
\hspace{3mm} \SummaryLLaMA{} & 0.574 & 0.433 & 0.453 & 0.01  & 0.01  & 0.01 \\
\hspace{3mm} \SummaryGPT{} & 0.634 & 0.524 & 0.546 & 0.09 & 0.02 & 0.03 \\
\hspace{3mm} \GSnip{} & 0.726 & 0.628 & \textbf{0.645} & 0.92 & 0.15 & \textbf{0.22} \\
\bottomrule
\end{tabular}
}

\vspace{-0.3em}
\caption{Prompting performance of \GPTFourMini{} across two classification tasks. The upper row shows the baseline (Prompting), and the lower block shows results with additional descriptive context. Best F1 values are bolded.}
\label{tab:gpt4o_prompting}
\vspace{-0.4em}
\end{table}

%...............................................................


Table~\ref{tab:gpt4o_prompting} shows that prompting \GPTFourMini{} yields only a 46.8\% F1 score for classifying organizations with respect to SIC codes. This result indicates that \GPTFourMini{} has not memorized the SIC codes from its pretraining data, so this is not a trivial task even for such a large language model. 

When we add the acquired text content to the prompt, Table~\ref{tab:gpt4o_prompting} reveals mixed results.  Adding \SummaryLLaMA{} does not improve performance. But adding \SummaryGPT{} does, achieving a 54.6\% F1 score, and adding \GSnip{} achieves a 64.5\% F1 score with substantial gains in both precision and recall over the prompting baseline.
% , approximately 18\% higher than the prompting baseline. 
These findings indicate that prompting alone is insufficient to solve this task, but augmenting the prompt with retrieved text, especially Google snippets, can substantially improve performance. %It proves particularly beneficial for rare entities, where the model’s parametric memory alone may be insufficient for accurate classification.

% \vspace{-0.8em}
\subsection{Classifier Experiments}
Table~\ref{tab:ft_with_LLMsumm} shows the performance of classifiers produced by fine-tuning different language models  using either \SummaryGPT{} or \SummaryLLaMA{} as the acquired text. All four models that use \SummaryGPT{} outperform those that use \SummaryLLaMA{}. The fine-tuned \GPTFourMini{} model with \SummaryGPT{} achieves the best result (66.4\% F1) and outperforms the best prompting result (64.5\% F1).
%..............................................
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{0.95}
\setlength{\tabcolsep}{2.8pt}

\resizebox{\columnwidth}{!}{
\begin{tabular}{@{\extracolsep{2pt}}lrrrrrr}
\toprule
Setting & \multicolumn{3}{c}{SIC Code} & \multicolumn{3}{c}{Healthcare Taxonomy} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& P & R & F1 & P & R & F1 \\
\midrule
BERT \\[-1pt]
\hspace{3mm} \SummaryLLaMA{} & 0.490 & 0.513 & 0.480 & 0.106 & 0.185 & 0.121 \\
\hspace{3mm} \SummaryGPT{}   & 0.562 & 0.560 & 0.532 & 0.143
 & 0.173 & 0.118 \\
\midrule
RoBERTa \\[-1pt]
\hspace{3mm} \SummaryLLaMA{} & 0.525 & 0.512 & 0.483 & 0.096 & 0.175 & 0.092 \\
\hspace{3mm} \SummaryGPT{}   & 0.581 & 0.565 & 0.550 & 0.222 & 0.189 & 0.139 \\
\midrule
Longformer \\[-1pt]
\hspace{3mm} \SummaryLLaMA{} & 0.512 & 0.515 & 0.481 & 0.055 & 0.069 & 0.049 \\
\hspace{3mm} \SummaryGPT{}   & 0.586 & 0.586 & 0.581 & 0.162 & 0.169 & 0.089 \\
\midrule
GPT-4o-mini \\[-1pt]
\hspace{3mm} \SummaryLLaMA{} & 0.657 & 0.648 & 0.649 & 0.187 & 0.219 & 0.191 \\
\hspace{3mm} \SummaryGPT{}   & 0.673 & 0.663 & \textbf{0.664} & 0.249 & 0.237 & \textbf{0.221} \\
\bottomrule
\end{tabular}
}

\vspace{-0.3em}
\caption{Fine-tuning performance across two classification tasks using LLM-generated summaries (\SummaryLLaMA{} and \SummaryGPT{}). Each block represents a fine-tuned model, and the best F1 values are bolded.}
\label{tab:ft_with_LLMsumm}
\vspace{-0.4em}
\end{table}

%...............................................


In the next set of experiments, we fine-tuned LLMs using the aggregated Google Snippets (\GSnip{}) as the acquired text. 
Table~\ref{tab:ft_with_gsnip_summary} shows these results, coupled with the \SummaryGPT{} results repeated from Table~\ref{tab:ft_with_LLMsumm} for direct comparison. The Google Snippets consistently outperform the LLM-generated summaries by a substantial margin. BERT, RoBERTa, Longformer and \GPTFourMini{} achieve absolute F1 scores gains of 17.2\%, 19.1\%, 16.5\%, and 15.3\%, respectively, compared to their counterparts that use \SummaryGPT{}. 
% \GPTFourMini{} also benefited significantly, achieving an F1 score of 81.7\%---a 15.3\% improvement over its \SummaryGPT{}-based fine-tuning, outperforming all other fine-tuned models.
%....................................................
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{0.95}
\setlength{\tabcolsep}{2.8pt}

\resizebox{\columnwidth}{!}{
\begin{tabular}{@{\extracolsep{2pt}}lrrrrrr}
\toprule
Setting & \multicolumn{3}{c}{SIC Code} & \multicolumn{3}{c}{Healthcare Taxonomy} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& P & R & F1 & P & R & F1 \\
\midrule
BERT \\[-1pt]
\hspace{3mm} \SummaryGPT{} & 0.562 & 0.560 & 0.532 & 0.143 & 0.173 & 0.118 \\
\hspace{3mm} \GSnip{} & 0.700 & 0.699 & 0.699 & 0.555 & 0.508 & 0.485 \\
\hspace{3mm} \GSnip{} + \SummaryGPT{} & 0.724 & 0.718 & 0.700 & 0.738 & 0.679 & 0.687 \\
\midrule
RoBERTa \\[-1pt]
\hspace{3mm} \SummaryGPT{} & 0.581 & 0.565 & 0.550 & 0.222 & 0.189 & 0.139 \\
\hspace{3mm} \GSnip{} & 0.757 & 0.748 & 0.741 & 0.688 & 0.608 & 0.604 \\
\hspace{3mm} \GSnip{} + \SummaryGPT{} & 0.774 & 0.769 & 0.763 & 0.742 & 0.683 & 0.693 \\
\midrule
Longformer \\[-1pt]
\hspace{3mm} \SummaryGPT{} & 0.586 & 0.586 & 0.581 & 0.162 & 0.169 & 0.089 \\
\hspace{3mm} \GSnip{} & 0.754 & 0.754 & 0.746 & 0.707 & 0.634 & 0.643 \\
\hspace{3mm} \GSnip{} + \SummaryGPT{} & 0.767 & 0.758 & 0.750 & 0.693 & 0.689 & 0.694 \\
\midrule
GPT-4o-mini \\[-1pt]
\hspace{3mm} \SummaryGPT{} & 0.673 & 0.663 & 0.664 & 0.249 & 0.237 & 0.221 \\
\hspace{3mm} \GSnip{} & 0.823 & 0.818 & 0.817 & 0.742 & 0.725 & \textbf{0.728} \\
\hspace{3mm} \GSnip{} + \SummaryGPT{} & 0.826 & 0.822 & \textbf{0.822} & 0.717 & 0.703 & 0.705 \\
\bottomrule
\end{tabular}
}

\vspace{-0.3em}
\caption{Fine-tuning performance across two classification tasks using different types of acquired text: LLM-generated summaries (\SummaryGPT{}), retrieved Google snippets (\GSnip{}), and their combination. Best F1 values are bolded.}
\label{tab:ft_with_gsnip_summary}
\vspace{-0.4em}
\end{table}


%....................................

Finally, we hypothesized that the LLM-generated summary and Google Snippets could provide complementary information and therefore both be valuable. So we also experimented with providing both types of information to the models by 
concatenating the \GSnip{} and \SummaryGPT{} texts.\footnote{We also tried combining \GSnip{} and \SummaryLLaMA{}. Performance was comparable to \GSnip{}+\SummaryGPT{}. %across all models. However, since it did not yield further improvements beyond the \SummaryGPT{} combination in any case, we exclude those results from the table for clarity and conciseness.
} The $GSnip+Summary_1$ rows in Table~\ref{tab:ft_with_gsnip_summary} show that this combined text yielded further performance gains for all models except BERT. Notably, this configuration of \GPTFourMini{} outperforms all other models with the best F1 score of 82.2\%.


\section{Analysis}
We conduct several analyses to gain insight into the performance and design choices of our framework.

\subsection{Why do Google Snippets outperform LLM summaries?}

Our first analysis investigates why Google Snippets performed better than  LLM-generated summaries (specifically, \SummaryGPT{}). We manually looked at 25 instances for which  \SummaryGPT{} led to an incorrect label but  \GSnip{} produced the correct label. 

In four cases, \GPTFourMini{} did not produce any summary (e.g., {\it ``I don’t have current detailed information \dots''}), leaving the model with no usable context so predictions were essentially arbitrary. 
% For instance, \textit{DGI RESOLUTION INC} was misclassified as \textit{Business Services (23)}, 
However, Google returned information that supported the correct label. 
% \GSnip{} provided information from multiple sources that supported the correct classification as \textit{Engineering, Accounting, Research (26)}. 
This finding shows that LLMs cannot always provide information about specific real-world entities if those entities are rare.

The most interesting issue pertains to the semantic framing of LLM-generated summaries. The summaries sometimes mentioned many things and included highly relevant information alongside tangential information. 
% For example, \textit{Gold Hill Resources, Inc.} was labeled as \textit{Metal Mining (0)} due to a summary emphasizing mining leadership, but \GSnip{} revealed its focus on wholesale, leading to the correct label \textit{Wholesale Trade – Durable Goods (12)}.
For example, \SummaryGPT{} emphasized secondary activities for \textit{SPARTON CORP}, such as medical instrumentation, resulting in a \textit{Measuring, Photographic, Medical (9)} label instead of the correct \textit{Electronic (7)} label. Similarly, \textit{AmREIT Monthly Income \& Growth Fund IV LP} was misclassified as \textit{Real Estate (20)} due to the absence of financial and investment context, which was present in \GSnip{} and led to the correct label \textit{Holding and Investment Offices (21)}.

% Moreover, blended or multi-domain descriptions in \SummaryGPT{} introduced ambiguity. For \textit{HORSESHOE GAMING LLC}, the inclusion of hospitality alongside recreation caused a shift toward \textit{Hotels and Camps (22)}, whereas \GSnip{}'s more focused recreational framing led to the correct label \textit{Amusement and Recreation Services (24)}.

% We also observe frequent confusion in semantically adjacent categories, especially where domain boundaries are subtle. \textit{REDDY ICE CORP} was incorrectly predicted as \textit{Wholesale – Nondurable Goods (13)} based on \SummaryGPT{}, while \GSnip{} more clearly framed its operations within the \textit{Food and Kindred Products (2)} category.

Overall, the summaries produced by \GPTFourMini{} were coherent and fluent but often presented a broad narrative that omitted the most relevant operational information. In contrast, \textit{GSnip} returned Web content that usually focused on the most salient facts. Aggregating 10 snippets also provided more semantically diverse content that enhanced robustness. 

% \vspace{-0.5em} 

\subsection{Performance across Categories}
\begin{figure*}[ht]
  \centering
  \includegraphics[width=\textwidth]{latex/figure/New-GSnipVsGSnip+GPT_f1_comparison_sorted.pdf}
  \caption{F1 scores across 27 SIC categories for \GPTFourMini{} fine-tuned with \GSnip{} vs. \GSnip{}+\SummaryGPT{}.}
  \label{fig:f1_comparison}
\end{figure*}
Figure~\ref{fig:f1_comparison} shows the F1 scores for each SIC category individually, for two of our models:  \GPTFourMini{} using \GSnip{} or using \GSnip{}+\SummaryGPT{}. The X-axis displays the categories, and the Y-axis shows the F1 scores. Each category is color-coded: green indicates categories where the combined text (\GSnip{}+\SummaryGPT{}) outperforms \GSnip{} alone, and red indicates where \GSnip{} yields better performance. These results show that 17 of the 27 categories benefitted from using both the LLM-generated summaries and the Google Snippets. 

Overall, performance varies across categories. Some lower-performing categories are challenging due to their generality (e.g., \textit{Miscellaneous Retail} and \textit{Business Services}), while others require fine-grained semantic distinctions (e.g., there are distinct categories for Wholesale Trade of Durable vs. Nondurable Goods).

%  Out of the 27 SIC categories:
% \begin{itemize}
% \item \textbf{17 categories} showed improved F1 scores when % \SummaryGPT{} was added to \GSnip{},
% \item \textbf{10 categories} experienced a performance decrease.
% \end{itemize}


% Although the majority of categories benefit from the combined input, some exhibit performance degradation, which is slight in most cases. However, three categories—\textit{Electronic}, \textit{Wholesale Trade – Nondurable Goods}, and \textit{Miscellaneous Retail}—experience more noticeable drops in performance. Upon analysis, we observed that \SummaryGPT{}  introduces terms that lead to misclassification. For example, organizations in the \textit{Electronic} category are sometimes misclassified as \textit{Chemicals and Allied Products}, \textit{Measuring, Photographic, Medical}, or \textit{Miscellaneous Retail}. Similarly, \textit{Wholesale Trade – Nondurable Goods} is often confused with \textit{Wholesale Trade – Durable Goods}, \textit{Eating and Drinking Places}, or \textit{Miscellaneous Retail}. These misclassifications likely occur because these categories are semantically related and involve overlapping business activities. Unlike \GSnip{},  \SummaryGPT{} may emphasize only a single aspect of an organization’s operations, potentially leading to ambiguity. Nonetheless, the overall trend indicates that most categories benefit from combining both sources.
%These results demonstrate that incorporating both retrieved and generated contextual information yields more accurate predictions in a majority of cases. The performance gains are particularly notable in categories where retrieved snippets alone may be sparse or noisy, indicating that \SummaryGPT{} helps reinforce and clarify relevant context. 
% \vspace{-0.5em}

\subsection{Why Top-10 Google Snippets?}
We also evaluated performance using different numbers of Google snippets to assess their impact on the results.
Table~\ref{tab:gpt4o_ablationStudy} shows that using multiple snippets improves performance up to a point: the F1 score increases steadily from top-1 to top-10, peaking at \textbf{0.817}. Beyond that, additional snippets provide diminishing returns and may even degrade performance, likely due to noise or redundancy.
%These findings reinforce that 10 snippets  offers the best tradeoff between informativeness and relevance.
\begin{table}[h]
    \centering
    \small
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{8pt} % Reduce column spacing
    \begin{tabular}{lccc}
        \hline
        \textbf{Fine-tuned \GPTFourMini{}} & \textbf{P} & \textbf{R} & \textbf{F1} \\
        \hline
        Top-1 snippet  & 0.691 & 0.687 & 0.686 \\
        Top-5 snippets  & 0.771 & 0.768 & 0.768 \\
        Top-10 snippets & \textbf{0.823} & \textbf{0.818} & \textbf{0.817} \\
        Top-15 snippets & 0.779 & 0.776 & 0.777 \\
        Top-20 snippets & 0.813 & 0.811 & 0.810 \\
        \hline
    \end{tabular}
    \caption{Performance of \GPTFourMini{} across different numbers of retrieved Google snippets.}
    \label{tab:gpt4o_ablationStudy}
    \vspace{-1em}
\end{table}
% \vspace{-1.1em}

\subsection{High Precision Categorization}
Ultimately, our goal is develop classification models that can be used to rapidly populate knowledge resources with task-specific information about real-world entities. Our best classification model achieved 82.6\% precision, which is  good. But ideally we would like even higher precision so that some instances can be labeled fully automatically without the need for human inspection. 

Toward this end, we experimented with  confidence thresholds to effect a trade-off between precision and recall. This approach considers the confidence of each label predicted by the classifier and only assigns the label if the confidence  exceeds a threshold. Our best classifiers used  GPT-4o mini,  but it  does not provide built-in support to extract confidence scores or log probabilities.
% from the GPT endpoint, we could not apply confidence-based analysis to this model. 
So we ran these experiments with  RoBERTa and Longformer.
%, which also have the advantage of being free to use. 

\begin{figure}[ht]
\vspace{-0.8em} 
  \centering  \includegraphics[width=\columnwidth, 
  trim=70 58 70 20, clip]{latex/figure/finalLR.pdf}
  %\vspace{-0.5em} 
  \caption{Precision/Recall trade-off curves for Longformer and RoBERTa based on confidence thresholds.}
  \label{fig:LR_recallPrecision}
  % \vspace{-0.8em}
\end{figure}

Figure~\ref{fig:LR_recallPrecision} displays the results. The squares in the lower right corner show the performance of RoBERTa and Longformer when labeling every instance (no threshold). The other data points show their performance using threshold values ranging from .60 to .85 in increments of five. 
Longformer's confidence scores proved more reliable than RoBERTa's, producing stronger high-precision results.  

This strategy successfully produced high precision ($>$ 90\%) classification while sacrificing some recall. For example, with a threshold of 0.85, Longformer achieved 96\% precision with around 30\% recall; using 0.60, it reached 91\% precision with 60\% recall. These high-precision classifiers  allow for fully automatic knowledge population for the most confident predictions.





==> latex/tables/table_GPTPerformance.tex <==
\begin{table}[h]
  \centering
  \renewcommand{\arraystretch}{1.2} 
  \setlength{\tabcolsep}{6pt}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l c c c}
      \specialrule{1.5pt}{0pt}{0pt} % Bold top border
      \textbf{Settings} & \textbf{P} & \textbf{R} & \textbf{F1 Score} \\
      \midrule % Thin line after heading
      \textit{GPT-4o mini } \\ 
      \hspace{5mm} Prompting  & 0.457 & 0.457 & 0.457 \\
      \hspace{5mm} Prompting (w/ GSnip) & \textbf{0.646} & \textbf{0.646} & \textbf{0.646} \\
      
      \specialrule{1.5pt}{0pt}{0pt} % Bold bottom border
    \end{tabular}
  }
  \caption{Performance comparison of GPT-4o mini under different settings.}
  \label{tab:gpt_performance}
\end{table}

\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.2} 
    \setlength{\tabcolsep}{12pt} % Adjust column spacing
    \begin{tabular}{l c c}
        \hline
        & P & R \\
        \hline
        Longformer & 0.770 & 0.755 \\
        RoBERTa & \textbf{0.776} & \textbf{0.765}\\
        \hline
    \end{tabular}
    \caption{Performance comparison of models based on Precision and Recall.}
    \label{tab:precision_recall_LR}
\end{table}

==> latex/tables/table_fineTunedModelPerformance.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{3pt} % Reduce spacing further
    \resizebox{\linewidth}{!}{ % Dynamically adjust table width
    \begin{tabular}{l>{\centering\arraybackslash}p{1.4cm} >{\centering\arraybackslash}p{1.4cm} >{\centering\arraybackslash}p{1.8cm}}
        \toprule
        \multicolumn{1}{c}{} & \multicolumn{3}{c}{F1 Score} \\
        \cmidrule(lr){2-4}
        & GPTSum & GSnip & \shortstack{GPTSum \\ + GSnip} \\
        \midrule
        \textit{BERT} & 0.555 & \textbf{0.717} & 0.715 \\
        \textit{RoBERTa} & 0.547 & 0.741 & \textbf{0.762} \\
        \textit{Longformer} & \textbf{0.563} & \textbf{0.745} & 0.749 \\
        \bottomrule
    \end{tabular}
    }
    \caption{F1 score comparison of different models under various settings.}
    \label{tab:performance}
\end{table}

